From Moderation to Mediation: Can LLMs Serve as Mediators in Online Flame Wars?

The rapid advancement of large language models (LLMs) has opened new possibilities for AI for good applications. As LLMs increasingly mediate online communication, their potential to foster empathy and constructive dialogue becomes an important frontier for responsible AI research. This work explores whether LLMs can serve not only as moderators that detect harmful content, but as mediators capable of understanding and de-escalating online conflicts. Our framework decomposes mediation into two subtasks: judgment, where an LLM evaluates the fairness and emotional dynamics of a conversation, and steering, where it generates empathetic, de-escalatory messages to guide participants toward resolution. To assess mediation quality, we construct a large Reddit-based dataset and propose a multi-stage evaluation pipeline combining principle-based scoring, user simulation, and human comparison. Experiments show that API-based models outperform open-source counterparts in both reasoning and intervention alignment when doing mediation. Our findings highlight both the promise and limitations of current LLMs as emerging agents for online social mediation.

==> introduction_v2.tex <==
In this work, we'll be exploring the use of LLM-as-a-Judge in the context of \textit{flame wars}. A flame war is an extended and heated exchange of hostile or insulting messages between individuals or groups in an online environment. The absence of face-to-face interaction reduces social restraint and encourages extreme expressions of anger or frustration~\cite{kiesler1984social}. Hostility is further provoked via social identity dynamics and the inherent anonymity in the exchange~\cite{Reicher01011995}. Flame wars usually progress in three phases~\cite{moor2010flaming}: 1) a trigger that often involves a perceived norm violation, 2) amplification through reciprocal hostility, and 3) entrenchment marked by topic abandonment. The final phase is characterized with ad-hominem loops that continue until participant fatigue sets in. Computational approaches have achieved reasonable success at detecting flame wars~\cite{steinberger2017flames}, but current systems remain mostly reactive, with emphasis on content removal or user suspension post hostility rather than constructive resolution as the situation is evoling. Political and identity-related discussions are especially susceptible to escalation, which can poison discourse and silence minority voices \cite{koiranen2022political, lee2005flaming, moor2010flaming}.

Our work aims to explore a different approach to intervention: mediation rather than moderation. Instead of asking whether a message is harmful, we ask whether an LLM can understand the flow of a conflict and intervene in ways that reduce tension. To do this, we view LLMs as potential mediators that can interpret multi-turn conversations, evaluate the fairness and relevance of the arguments being made, and generate responses that acknowledge concerns, reduce hostility, and guide the exchange toward a more constructive path. This requires reasoning about context, emotion, escalation patterns, and conversational norms \cite{REF NEEDED}. To achieve this goal, we divide the task into two complementary components. The first is judgment, where an LLM evaluates the interaction and identifies unfair claims, emotional triggers, and points of escalation. The second is steering, where the model produces a message aimed at calming the exchange and helping participants refocus on their actual disagreement instead of attacking each other. These two subtasks build on the broader literature on LLM-as-a-judge, but they extend it to a dynamic social setting where the goal is to guide people toward resolution rather than simply score a message.

Towards mitigating flame wars, we developed a \textit{principle-based evaluation framework} for interactive mediation: we use conversation-derived principles to assess both judgment (evaluative reasoning) and steering (de-escalatory guidance). This extends LLM-as-a-Judge beyond rigid moderation into active, context-sensitive social reasoning and mediation. To do this, we view LLMs as potential mediators that can interpret multi-turn conversations, evaluate the fairness and relevance of the arguments being made, and generate responses that acknowledge concerns, reduce hostility, and guide the exchange toward a more constructive path. Specifically, we divide the task into two complementary components. The first is judgment, where an LLM evaluates the interaction and identifies unfair claims, emotional triggers, and points of escalation. The second is steering, where the model produces a message aimed at calming the exchange and helping participants refocus on their actual disagreement instead of attacking each other. Both components require reasoning about context, emotion, escalation patterns, and conversational norms \cite{REF NEEDED}. If successful, this architecture will guide people toward resolution rather than simply scoring messages.

Our main contributions are summarized as follows:
\begin{itemize}
    \item[\ding{182}] We introduce the first comprehensive framework for LLM-based mediation in online flame wars, covering both judgment and steering subtasks.
    \item[\ding{183}] We construct a new dataset of multi-turn adversarial Reddit conversations designed specifically for mediation research.
    \item[\ding{184}] We propose a principle-based evaluation protocol that integrates LLM-as-a-judge reasoning, user simulation, and human assessment.
    \item[\ding{185}] We provide empirical insights into how LLMs respond to conflictual discourse and where they succeed or fail as mediators.
\end{itemize}
